Multivariate Time Series Forecasting with Latent Graph Inference

This paper introduces a new approach for Multivariate Time Series forecasting that jointly infers and leverages relations among time series. Its modularity allows it to be integrated with current univariate methods. Our approach allows to trade-off accuracy and computational efficiency gradually via offering on one extreme inference of a potentially fully-connected graph or on another extreme a bipartite graph. In the potentially fully-connected case we consider all pair-wise interactions among time-series which yields the best forecasting accuracy. Conversely, the bipartite case leverages the dependency structure by inter-communicating the N time series through a small set of K auxiliary nodes that we introduce. This reduces the time and memory complexity w.r.t. previous graph inference methods from O(N^2) to O(NK) with a small trade-off in accuracy. We demonstrate the effectiveness of our model in a variety of datasets where both of its variants perform better or very competitively to previous graph inference methods in terms of forecasting accuracy and time efficiency.

==> ICML - Time Series Forecasting (6)/sections/background.tex <==
%%!TEX root = ../example_paper.tex

\section{Background}


\subsection{Time Series Forecasting} \label{sec:background_tsf}

In time series forecasting we aim to estimate a future time series $\rmx_{t+1:T}$ given its past $\rmx_{t_0:t}$ where $t_0 \leq t \leq T$ indexes over time, and (optionally) some context information $\rmc$. For the multivariate case we assume the time series is composed of $N$ variates at a time such that $\rmx_{t_0:T} = \{\rmx_{1, t_0:T}, \dots, \rmx_{N, t_0:T}\} \in \mathbb{R}^{N \times T-t_0+1}$. In this section we distinguish two main categories of time series forecasting methods, Global Univariate and Multivariate.

\textbf{Global Univariate methods}: In this case we only use the past of each univariate to predict its future. However, the model weights $\theta_u$ are shared across all univariate time series. More formally:
\begin{equation} \label{eq:univariate}
    \hat{\rmx}_{i,t+1:T} = f_{u}(\rmx_{i,t_0:t}, \rmc_i; \theta_u)
\end{equation}
where $\hat{\rmx}$ denotes the estimated values, $i \in \{1, \dots, N\}$ indexes over multivariates and $f_{_u}(\cdot)$ is the estimator function with learnable parameters $\theta_u$ shared across time series. Conditioning on the past of each univariate may limit the performance of the forecasting algorithm compared to multivariate ones. Despite that, it simplifies the design of $f_\theta$ and already provides reasonable results. A popular example of a global univariate model is DeepAR~\citep{salinas2020deepar}.


\textbf{Multivariate methods}: Multivariate methods condition on all past data (all $N$ variates) and directly predict the multivariate target. More formally:
\begin{equation}
    \hat{\rmx}_{t+1:T} = f_{m}(\rmx_{t_0:t}, \rmc).
\end{equation}
Different variables may be correlated and/or depend on the same con-founders. For example, in retail forecasting, PPE masks and antibacterial soaps jointly increased in demand during the early days of the COVID-19 pandemic. In traffic forecasting, an increase of the outcome traffic flow in a given neighborhood may result in an increase of the income traffic flow on another one. Modelling these dependencies may improve the forecasting accuracy, but it may come at a cost of higher complexity and hence more expensive algorithms, especially when trying to model all pairwise interactions between variates.


\subsection{Graph Neural Networks} \label{sec:background_gnns}
Graph Neural Networks (GNNs) \citep{bruna2013spectral, defferrard2016convolutional, kipf2016semi} operate directly on graph structured data. They have gained a lot of attention in the last years due to their success in a large variety of domains which benefit from modelling interactions between different nodes/entities. In the context of multivariate time series, GNNs can be used to model the interactions between time series. In this work we consider the type of GNN introduced by \citep{gilmer2017neural}. Given a graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ with nodes $v_i \in \mathcal{V}$ and edges $e_{ij} \in \mathcal{E}$,  we define a graph convolutional layer as:
\begin{equation} \label{eq:gnn}
\small
    \rmm_{ij} = \phi_e(\rmh_i^l, \rmh_j^l), 
\qquad
%\rmm_i = \sum_{j \in \mathcal{N}(i)} \alpha_{ij}\rmm_{i j},
%\quad
\rmh_i^{l+1} = \phi_h(\rmh_i^l, \sum_{j \in \mathcal{N}(i)} \alpha_{ij}\rmm_{i j}) 
\end{equation}
%\begin{align}
%\rmm_{ij} &= \phi_e(\rmh_i^l, %\rmh_j^l) \label{eq:gnn_message}\\
%    \rmm_i &= \sum_{j \in \mathcal{N}(i)} \alpha_{ij}\rmm_{i j} \label{eq:gnn_aggr} \\ 
%    \rmh_i^{l+1} &= \phi_h(\rmh_i^l, \rmm_i) \label{eq:gnn_node}
%\end{align}
Where $\phi_e$ and $\phi_h$ are the edge and node functions, usually approximated as Multi Layer Perceptrons (MLPs), $\rmh^l_i \in \mathbb{R}^{\text{nf}}$ is the nf-dimensional embedding of a node $v_i$ at layer $l$ and $\rmm_{ij}$ is the edge embedding that propagates information from node $v_j$ to $v_i$. A GNN is constructed by stacking multiple of these Graph Convolutional Layers $\rmh^{l+1} = \mathrm{GCL}[\rmh^{l}, \mathcal{E}]$. Additionally, in~\shorteqref{eq:gnn} we include $\alpha_{ij} \in (0,1)$ which is a scalar value that performs the edge inference or attention over the neighbors similarly to~\cite{velivckovic2017graph}. Following~\citep{satorras2021n}, we choose this value to be computed as the output of a function $\alpha_{ij}=\phi_\alpha(\rmm_{ij})$ where $\phi_\alpha$ is composed of just a linear layer followed by a sigmoid activation function.

==> ICML - Time Series Forecasting (6)/sections/conclusions.tex <==
%%!TEX root = ../example_paper.tex

\section{Conclusions}
We presented a novel approach for multi-variate time series forecasting which lends itself to easy integration into existing univariate approaches by ways of a graph neural network (GNN) component. This GNN infers a latent graph in the space of the embeddings of the univariate time series and can be inserted in many neural-network based forecasting models. We show that this additional graph/dependency structure improves forecasting accuracy both in general and in particular when compared to the state of the art. We alleviate typical scalability concerns for GNNs via allowing the introduction of auxiliary nodes in the latent graph which we construct as a bipartite graph that bounds the computational complexity. We show that this leads to computationally favorable properties as expected while the trade-off with forecasting accuracy is manageable. 

==> ICML - Time Series Forecasting (6)/sections/experiments.tex <==
%%!TEX root = ../example_paper.tex

\section{Experiments} \label{sec:experiments}
%In this section we evaluate the accuracy and complexity of our model in a wide variety of datasets. We show our work performs competitively or better than previous works while being more efficient in running time.
\subsection{Datasets and Baselines}


\begin{table}[h!]
\vspace{-5pt}
\scriptsize
%\setlength{\tabcolsep}{3.5pt}
\begin{center} 
\begin{tabular}{l | cc cc  }
\toprule
 & \#Nodes & \# Samples & Context length & Pred. length\\
 \midrule
 METR-LA & 207 & 34,272 & 12 & 12 \\
PEMS-BAY & 325 & 52,116 & 12 & 12 \\
\midrule
Solar-Energy & 137 & 52,560 & 168 & 1\\
Traffic & 862 & 17,544 & 168 & 1\\
Electricity & 321 & 26,304 & 168 & 1\\
Exchange-Rate & 8  &  7,588 & 168 & 1\\
    \bottomrule
\end{tabular}
\vspace{-5pt}
\caption{Dataset specifications.}
\label{tab:mtgnn_results} 
\label{table:datasets}
\end{center}
%\end{table}
%\vspace{-10pt}
\vspace{-15pt}
\end{table}

We first evaluate our method on METR-LA and PEMS-BAY datasets~\citep{li2017diffusion} which record traffic speed statistics on the highways of Los Angeles county and the Bay Area respectively. %They are intrinsically structured over a city which makes them suitable for latent graph inference.  
We also consider the publicly available Solar-Energy, Traffic, Electricity and Exchange-Rate data sets. Specifications for each dataset are presented in Table \ref{table:datasets} and further detailed in Appendices \ref{ap:metr_pems} and \ref{ap:single_step_impl_details}.
%where \#Nodes is the number of time series in the panel, \#Samples is the number of time steps in each time series, Context length is the length of the input window and Pred. Length is the length of the predicted window. 
%We compare to a variety of baselines including previous works and variations of our proposed method. We distinguish the following three main types of baselines (Univariate, Multivariate with known graph and Multivariate with graph inference):
We compare to the following three main types of baselines:


\begin{table*}[t]
\scriptsize
\setlength{\tabcolsep}{3.5pt}
\begin{center}
\begin{tabular}{l | ccc | ccc | ccc | ccc | ccc | ccc  }
\toprule
 & \multicolumn{9}{c|}{METR-LA} & \multicolumn{9}{c}{PEMS-BAY}  \\
 & \multicolumn{3}{c}{15 min} & \multicolumn{3}{c}{30 min} & \multicolumn{3}{c|}{60 min}& \multicolumn{3}{c}{15 min} & \multicolumn{3}{c}{30 min} & \multicolumn{3}{c}{60 min} \\
 \midrule
  & \tiny MAE & \tiny RMSE & \tiny MAPE & \tiny MAE & \tiny RMSE & \tiny MAPE & \tiny MAE & \tiny RMSE & \tiny MAPE & \tiny  MAE & \tiny RMSE & \tiny  \tiny MAPE & \tiny MAE & \tiny RMSE & \tiny MAPE & \tiny MAE & \tiny RMSE & \tiny MAPE \\
 \midrule
x5 Linear / AR & 3.81 & 8.80 & 9.13\% & 4.94 & 11.14 & 12.17\% & 6.30 & 12.91 & 16.72\% & 1.59 & 3.41 & 3.27\% &  2.15 & 4.87 & 4.77 \% & 2.97 & 6.65 & 7.03\% \\
 \midrule

 DCRNN & 2.77 & 5.38 & 7.30\% & 3.15 & 6.45 & 8.80\% & 3.60 & 7.60 & 10.50\% & 1.38 & 2.95 & 2.90\% & 1.74 & 3.97 & 3.90\% & 2.07 & 4.74 & 4.90\% \\
 STGCN & 2.88 & 5.74 & 7.6\% & 3.47 & 7.24 & 9.6\% & 4.59 & 9.40 & 12.7\% & 1.36 & 2.96 & 2.9\% & 1.81 & 4.27 & 4.2\% & 2.49 & 5.69 & 5.8\%\\
 %GMAN & 2.77 & 5.48 & 7.25\% & 3.07 & 6.34 & 8.35\% & 3.40 & 7.21 & 9.72\% & 1.34 & 2.82 & 2.81\% & 1.62\% & 3.72 & 3.63\% & 1.86 & 4.32 & 4.31\% \\
 % GMAN & - & - & - & - & - & - & - & - & - & 1.34 & 2.82 & 2.81\% & 1.62 & 3.72 & 3.63\% & 1.86 & 4.32 & 4.31\% \\  I removed this one because it is very inconsistent with the paper
 MRA-BGCN & 2.67 & \textbf{5.12} & \textbf{6.8}\% & 3.06 & 6.17 & 8.3\% & 3.49 & 7.30 & 10.0\% & \textbf{1.29} & \textbf{2.72} & 2.9\% & \textbf{1.61} & \textbf{3.67} & 3.8\% & \textbf{1.91} & \textbf{4.46} & 4.6\% \\
 \midrule
   Graph WaveNet* & 2.69 & 5.15 & 6.90\% & 3.07 & 6.22 & 8.37\% & 3.53 & 7.37 & 10.01\% & 1.30 & 2.74 & \textbf{2.73\%} & 1.63 & 3.70 & \textbf{3.67\%} & 1.95 & 4.52 & 4.63\% \\
 LDS & 2.75 & 5.35 & 7.1\% & 3.14 & 6.45 & 8.6\% & 3.63 & 7.67 & 10.34\% & 1.33 & 2.81 & 2.8\% & 1.67 & 3.80 & 3.8\% & 1.99 & 4.59 & 4.8 \% \\
MTGNN & 2.69 & 5.18 & 6.86\% & 3.05 & 6.17 & 8.19\% & 3.49 & 7.23 & 9.87\% & 1.32 & 2.79 & 2.77\% & 1.65 & 3.74 & 3.69\% & 1.94 & 4.49 & \textbf{4.53}\%
  \\
    %GTS (official) & 2.64 & 4.95 & 6.8\% & 3.01  &  5.85 & 8.2\% & 3.41 &  6.74 & 9.9\% & 1.32 & 2.62 & 2.8\% & 1.64 & 3.41 & 3.6\% & 1.91 & 3.97 & 4.4\%  \\
        GTS & 2.64 & 5.19 & 6.79\% & 3.06 & 6.30 & 8.24\% & 3.56 & 7.55 & 9.95\% & 1.35& 2.84 & 2.85\% & 1.67 & 3.82 & 3.80\% & 1.96 & 4.53 & 4.62\% \\
     \midrule
       \textit{Ablation study} &    \\
 NE-GNN \textit{(w/o id)} & 2.80 & 5.73 & 7.50\% & 3.40 & 7.15 & 9.74\% & 4.22 & 8.79 & 13.06\% & 1.40 & 3.03 & 2.92\% & 1.85 & 4.25 & 4.21\% & 2.39 & 5.50 & 5.93\%  \\
 FC-GNN \textit{(w/o id)} & 2.77 & 5.65 & 7.39\% & 3.36 & 7.02 & 9.59\% & 4.14 & 8.64 & 12.70\% & 1.39 & 3.00 & 2.88\% & 1.82 & 4.18 & 4.11\% & 2.32 & 5.35 & 5.71\%  \\
 NE-GNN & 2.69 & 5.57 & 7.21\% & 3.14 & 6.74 & 9.01\% & 3.62 & 7.88 & 10.94\% & 1.36 & 2.88 & 2.86\% & 1.72 & 3.91 & 3.93 \% & 2.07 & 4.79 & 5.04\% \\
 \midrule
 \textit{Our models} & \\
 FC-GNN & \textbf{2.60} & 5.19 & \textbf{6.78\%} & \textbf{2.95} & \textbf{6.15} & \textbf{8.14\%} & \textbf{3.35} & \textbf{7.14} & \textbf{9.73\%} & 1.33 & 2.82 & 2.79\% & 1.65 & 3.75 & \textbf{3.72\%} & 1.93 & \textbf{4.46} & \textbf{4.53}\%    \\
  BP-GNN (K=4) & 2.64 & 5.37 & 7.07\% & 3.02 & 6.42 & 8.46\% &  3.40 & 7.32 & 9.91\% & 1.33 &  2.82 & 2.80\% & 1.66 & 3.78 & 3.75\% & 1.94 & \textbf{4.46} & 4.57\% \\
    \bottomrule
\end{tabular}
\caption{Benchmark on METR-LA and PEMS-BAY datasets. Mean Absolute Error (MAE), Root Mean Squared Error (RMSE) and Mean Absolute Percentage Error (MAPE) are reported for different time horizons \{15, 30, 60\} minutes. Results have been averaged over 5 runs.}
\vspace{-10pt}
\label{tab:overview_results}
\end{center}
\end{table*}


\begin{itemize}[leftmargin=*]
    \item Univariate: In this case a single model is trained for all time series but they are treated independently without message exchange among them. These baselines include a simple linear Auto Regressive model (AR) and a variation of our FC-GNN method that we called NE-GNN where all edges have been removed such that the aggregation function $\mathrm{AGG}$ becomes equivalent to a multilayer perceptron defined by $\phi_h$~\shorteqref{eq:gnn}. 
    \item Multivariate with a known graph: These methods require a previously defined graph, therefore they are restricted to those datasets where an adjacency matrix can be pre-defined (e.g. METR-LA, PEMS-BAY). From this group we compare to DCRNN \citep{li2017diffusion}, STGCN \citep{yu2017spatio} and MRA-BGCN \citep{chen2020multi}.
    
    \item Multivariate with graph inference or attention: These methods exchange information among different time series by simultaneously inferring relations among them or by attention mechanisms. From this group we compare to LDS \citep{franceschi2019learning},
    LST-Skip \citep{lai2018modeling}, TPA-LSTM \citep{shih2019temporal}, MTGNN \citep{wu2020connecting} and GTS \citep{shang2021discrete}. Graph WaveNet \citep{wu2019graph} also belongs to this group but unlike the others it jointly uses a pre-defined adjacency matrix. Comparisons to NRI \citep{kipf2018neural} can be found in previous literature \citep{shang2021discrete, zugner2021study}. We additionally include a variation of our FC-GNN without unique node ids, we denote it by \textit{(w/o id)} beside the model name. GTS numbers have been obtained by averaging over 3 runs its official implementation.
\end{itemize}



\subsection{Main results} \label{sec:main_results}


In this section we evaluate our method in METR-LA and PEMS-BAY datasets. For this experiment we used the training setup from GTS \citep{shang2021discrete} which uses the dataset partitions and evaluation metrics originally proposed in \citep{li2017diffusion}. All our models have been trained by minimizing the Mean Absolute Error (MAE) between the predicted and ground truth samples. The reported metrics are MAE, Root Mean Squared Error (RMSE) and Mean Absolute Percentage Error (MAPE) from \citep{li2017diffusion}. All metrics have been averaged over 5 runs. All our models (FC-GNN, BP-GNN and NE-GNN) contain 2 graph convolutional layers, 64 features in the hidden layers, Swish activation functions \citep{ramachandran2017searching} and have been trained with batch size 16. The number of auxiliary nodes in BP-GNN was set to $K=4$.  Time experiments report the average forward pass in seconds for a batch size 16 in a Tesla V100-SXM GPU. Further implementation details are provided in Appendix \ref{ap:impl_metr_pems}.





\textbf{Results} are reported in Tables \ref{tab:overview_results} and \ref{tab:time_results}, standard deviations in Appendix \ref{ap:metr_pems_std}.
FC-GNN outperforms other methods in most metrics while being computationally cheaper than previous works. On the other hand, BP-GNN performs very competitively w.r.t. previous works (even outperforming all previous methods in some metrics) but with a vast decrease in computation. Furthermore, these performances are achieved without explicitly providing the structural information of the city (i.e. pre-defined adjacency) unlike in those methods that require it (e.g. MRA-BGCN) or in Graph Wavenet that optionally uses it. Additionally, note the performance gap between FC-GNN and NE-GNN is larger when including a unique identifier of the nodes. This means the network can better leverage the information exchange among nodes when they are uniquely identified, but it still benefits from the message passing scheme when they are not uniquely identified (w/o id) thanks to the dynamical inference.
 %Finally, we want to point out that the spatial information of the city is only used in those methods that require a pre-defined adjacency matrix, but despite that, the performance doesn't vary that much compared to the graph inference methods.  %Finally, we want to point out that models like ours that infer the graph  not necessarily include the spatial information of the city required in those methods that need a pre-defined adjacency matrix used to compute the adjacency matrix in those methods that require it but they still perform better or very competitively.
 \begin{table}[h!]
\vspace{-5pt}
\footnotesize
%\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.9}
\begin{center}
\begin{tabular}{l | cc  }
\toprule
 & \multicolumn{2}{c}{Forward Time (s)} \\
 & METR-LA & PEMS-BAY \\
 \midrule
 Linear & .0002 & .0002\\
 \midrule
 DCRNN & .2559  & .2754 \\
 \midrule
 Graph WaveNet & .0500 & .0673\\
 MTGNN & .0160 & .0371\\
 GTS & .0869 & .1087\\
 \midrule
 NE-GNN & .0033 & .0047\\
 FC-GNN & .0108 & .0253\\
 BP-GNN (K=4) & .0044 & .0046\\
    \bottomrule
\end{tabular}
\vspace{-6pt}
\caption{Forward time in seconds for different methods.}
\label{tab:time_results}
\end{center}
%\end{table}
\vspace{-5pt}
\end{table}
Time results are reported in Table \ref{tab:time_results}. We include all methods from the previous Table \ref{tab:overview_results} that have a publicly available implementation in METR-LA and PEMS-BAY datasets. BP-GNN is the most efficient algorithm in both METR-LA and PEMS-BAY by a large margin. FC-GNN is also more efficient than previous methods in both datasets but it is still limited by the $O(N^2)$ scalability. In the next Section \ref{sec:single_step} we will see that BP-GNN becomes even more efficient for larger graphs compared to the other methods thanks to its better scalability. %A time  comparison with LDS is provided in \citep{shang2021discrete} where it is reported to be considerably slower than GTS and DCRNN.






%\begin{table}[h]

%\setlength{\tabcolsep}{2pt}


\begin{table*}[t]
\scriptsize
\setlength{\tabcolsep}{4pt}

\begin{center}
\begin{tabular}{ll | c | cccc | cccc | cccc | cccc}
\toprule
\multicolumn{2}{c|}{Dataset} &
&\multicolumn{4}{|c|}{Solar-Energy} & \multicolumn{4}{|c|}{Traffic} &
\multicolumn{4}{|c|}{Electricity} &
\multicolumn{4}{|c}{Exchange-Rate} \\
\midrule
\multicolumn{2}{c|}{} &
\multicolumn{1}{c|}{}&
\multicolumn{4}{c}{Horizon} & \multicolumn{4}{|c|}{Horizon} & \multicolumn{4}{|c|}{Horizon} & \multicolumn{4}{|c}{Horizon} \\
Methods & Metrics & \#Top2 &
3 & 6 & 12 & 24 &
3 & 6 & 12 & 24 &
3 & 6 & 12 & 24 &
3 & 6 & 12 & 24\\
\midrule
\multirow{2}{*}{AR} & RSE & (0) & .2435 & .3790 & .5911 & .8699 & .5991 & .6218 & .6252 & .6293 & .0995 & .1035 & .1050 & .1054 & .0228 & .0279 & .0353 & .0445 \\
& CORR & (0) & .9710 & .9263 & .8107 & .5314 & .7752 & .7568 & .7544 & .7519 & .8845 & .8632 & .8591 & .8595 & .9734 & .9656 & .9526 & .9357 \\
\multirow{2}{*}{RNN-GRU} & RSE & (0) & .1843 & .2559 & .3254 & .4643 & .4777 & .4893 & .4950 & .4973 & .0864 & .0931 & .1007 & .1007 & .0226 & .0280 & .0356 & .0449 \\
& CORR & (0)  & .9843 & .9690 & .9467 & .8870 & .8721 & .8690 & .8614 & .8588 & .9283 & .9135 & .9077 & .9119 & .9735 & .9658 & .9511 & .9354 \\
\multirow{2}{*}{LST-skip} & RSE & (0) & .1843 & .2559 & .3254 & .4643 & .4777 & .4893 & .4950 & .4973 & .0864 & .0931 & .1007 & .1007 & .0226 & .0280 & .0356 & .0449 \\
& CORR & (0) & .9843 & .9690 & .9467 & .8870 & .8721 & .8690 & .8614 & .8588 & .9283 & .9135 & .9077 & .9119 & .9735 & .9658 & .9511 & .9354 \\
\multirow{2}{*}{TPA-LSTM} & RSE & (3) & .1803 & .2347 & .3234 & .4389 & .4487 & .4658 & .4641 & .4765 & .0823 & .0916 & .0964 & .1006 & \textbf{.0174} & \textbf{.0241} & .0341 & \secondbest{.0444} \\
& CORR & (4)& .9850 & .9742 & .9487 & .9081 & .8812 & .8717 & .8717 & .8629 & .9439 & .9337 & .9250 & .9133 & \textbf{.9790} & \textbf{.9709} & \textbf{.9564} & \textbf{.9381} \\
\multirow{2}{*}{MTGNN} & RSE & (5) & .1778 & .2348 & .3109 & .4270 & .4162 & .4754 & \textbf{.4461} & \textbf{.4535} & .0745 & \textbf{.0878} & \secondbest{.0916} & \textbf{.0953} & .0194 & .0259 & .0349 & .0456 \\
& CORR & (6) & .9852 & .9726 & .9509 & .9031 & .8963 & .8667 & \textbf{.8794} & \textbf{.8810} & .9474 & .9316 & .9278 & .9234 & \secondbest{.9786} & \secondbest{.9708} & \secondbest{.9551} & \secondbest{.9372} \\
\midrule
\midrule
%\multirow{2}{*}{$\underset{\text{w/o id}}{\text{NE-GNN}}$} & RSE &  \\
%& CORR \\
\multirow{2}{*}{NE-GNN} & RSE & (2) & .1898 & .2580 & .3472 & .4441 & .4212 & .4586 & .4679 & .4743 & .0762 & .0917 & .0966 & .0994 & .0175 & \secondbest{.0244} & \textbf{.0338} & .0447 \\
& CORR & (0) & .9829 & .9663 & .9367 & .8905 & .8951 & .8748 & .8700 & .8670 & .9494 & .9362 & .9308 & .9262 & .9769 & .9686 & .9535 & .9352 \\
%\midrule
\multirow{2}{*}{FC-GNN} & RSE & \textbf{(12)} & \textbf{.1651} & \textbf{.2202} & \textbf{.2981} & \textbf{.3997} & \textbf{.4057} & \textbf{.4395} & \secondbest{.4624} & \secondbest{.4620} &  \textbf{.0732} & .0907 & \textbf{.0915} & \secondbest{.0979} & \textbf{.0174} & .0245 & .0344 & .0450  \\
& CORR & \textbf{(12)} & \textbf{.9876} & \textbf{.9765} & \textbf{.9551} & \textbf{.9148} & \textbf{.9024} & \textbf{.8850} & \secondbest{.8764} & \secondbest{.8751} & \textbf{.9521} & \textbf{.9404} & .\textbf{9351} & \textbf{.9294} & .9772 & .9685 & .9538 & .9349 \\
\multirow{2}{*}{$\underset{\text{(K=4)}}{\text{BP-GNN}}$} & RSE & (11) & \secondbest{.1704} & \secondbest{.2257} & \secondbest{.3072} & \secondbest{.4050} & \secondbest{.4095} & \secondbest{.4470} & .4640 & .4641 & \secondbest{.0740} & \secondbest{.0898} &  .0940 & .0980 & .0175 & \secondbest{.0244} & \secondbest{.0339} & \textbf{.0442}  \\
& CORR & (10) & \secondbest{.9865} & \secondbest{.9751} & \secondbest{.9522} & \secondbest{.9138}  & \secondbest{.8999} & \secondbest{.8820} & .8744 & .8723 & \secondbest{.9519} & \secondbest{.9396} & \secondbest{.9345} & \secondbest{.9288} & .9769 & .9684 & .9530 & .9360 \\
\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{Benchmark on Solar-Energy, Traffic, Electricity and Exchange-Rate. Root Relative Squared Error (RSE) and Empirical Correlation Coefficient (CORR) are reported for different horizons \{3, 6, 12, 24\}. All results have been averaged over 5 runs. \#Top2 column counts how many metrics in each row are in the top 2 (i.e. bold).  }
\label{tab:electricity_traffic}
\end{center}
\vspace{-5pt}
\end{table*}


\subsection{Single step forecasting} \label{sec:single_step}


In this section, we evaluate our method on the publicly avilable Solar-Energy, Traffic, Electricity and Exchange-Rate datasets. In contrast to METR-LA and PEMS-BAY, these datasets do not contain spatial information from which a graph can be pre-defined, therefore, methods that rely on a known graph are not directly applicable. To ensure comparability, we use the same training settings as \citep{lai2018modeling, shih2019temporal, wu2020connecting} in which the network is trained to predict one time step into the future (single step forecasting) with a given horizon (3, 6, 12, or 24) by minimizing the Mean Absolute Error (MAE). All datasets have been split in 60\%/20\%/20\% for training/val/test respectively. As proposed in \citep{lai2018modeling} we use the Root Relative Squared Error (RSE) and Empirical Correlation Coefficient (CORR) as evaluation metrics (both defined in Appendix \ref{ap:evaluation_metrics}). All our models (FC-GNN, BP-GNN and NE-GNN) contain 2 graph convolutional layers and 128 features in the hidden layers. The timing results have been obtained with batch size 16. Further implementation details are provided in Appendix~\ref{ap:single_step_impl_details}. Results with standard deviations are provided in Appendix~\ref{ap:single_step_std}.

% BP-GNN in batches of 2 for Traffic --> 0,0624


\textbf{Results} in Table \ref{tab:electricity_traffic} are consistent with the previous experiment. FC-GNN outperforms all previous works in most metrics. There is a significant improvement over NE-GNN, which demonstrates that sharing information among nodes is beneficial (except in Exchange-Rate dataset which only contains 8 nodes). BP-GNN performs better than previous methods in most metrics and close to FC-GNN. Regarding the timing results (Table \ref{tab:timing_results2}), BP-GNN is the most efficient graph inference method by a large margin in most datasets. 
The larger the number of nodes in the dataset, the larger the computational improvement of BP-GNN w.r.t. other methods due to its linear scalability when $K=4    $. 
\begin{table}[h!]
\footnotesize
%\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.0}

\begin{center}
\begin{tabular}{l | cccc  }
\toprule
 & Exchange & Solar & Electricity & Traffic \\
 \midrule
 \# Nodes & 8 & 137 & 321 & 862 \\
 \midrule
 MTGNN & .0062 & .0146 & .0771 & 1.1808\\
 \midrule
 NE-GNN & .0034 & .0059 & .0067 & .0117 \\
 FC-GNN & .0053 & .0109 & .0536 &  .4184\\
 BP-GNN & .0076 & .0076 & .0084 & .0121\\
    \bottomrule
\end{tabular}
\caption{Forward average time in seconds for different methods in Solar-Energy, Traffic, Electricity and Exchange-Rate datasets.}
\vspace{-5pt}
\label{tab:timing_results2}
\vspace{-15pt}
\end{center}
\end{table}
For example, in Solar-Energy (137 nodes), BP-GNN is 1.43 times faster than FC-GNN and 1.92 times faster than MTGNN. Accordingly, in a larger dataset as Electricity (321 nodes) BP-GNN is 6.38 times faster than FC-GNN and 9.18 times faster than MTGNN. In the largest dataset, Traffic (862 nodes), BP-GNN becomes 34.58 times faster than FC-GNN and 97.59 times faster than MTGNN, although in traffic, MTGNN and FC-GNN did not fit in the GPU for a batch of 16 (also because to the $O(N^2)$ complexity), and we had to pass the samples in batches of 2 which eliminates part of the GPU parallelization. Running BP-GNN in batches of 2, would result in it being 7.71 and 18.92 times faster than FC-GNN and MTGNN respectively. Finally, in such small graphs as Exchange Rate, there is no computational benefit in using the bipartite assumption since the number of edges for both the bipartite and the fully connected graphs becomes the same (for K=4 and N=8). 

%\subsection{Inferred graph analysis} %\label{sec:inferred_graph}
%\begin{figure*}[t]
%\center
%\includegraphics[width=0.6\%linewidth]{figures/inference_experiment.png}
%\vspace{-5pt}
%\caption{Inferred adjacency matrices and MAE losses in the proposed synthetic datasets.}
%\label{fig:inference_results}
%\vspace{-5pt}
%\end{figure*}

\subsection{Inferred graph analysis} \label{sec:inferred_graph}
\begin{figure}[t]
\center
\includegraphics[width=1\linewidth]{figures/inference_experiment_new.png}
\vspace{-20pt}
\caption{Inferred adjacency matrices and MAE losses in the proposed synthetic datasets for FC-GNN, BP-GNN and NE-GNN.}
\label{fig:inference_results}
\vspace{-15pt}
\end{figure}

In this section we study the adjacency matrices inferred by FC-GNN. For this purpose, we generated synthetic datasets with different numbers of nodes N and $T=10.000$ timesteps each. (a) "Cycle Graph" dataset samples each series value $\rmx_{i,t}$ from the past $(t-5)$ of another series $(i-1 \mod N)$ from the panel. The resulting adjacency matrix is a directed cycle graph. More formally, the dataset is generated from the following gaussian distribution $\rmx_{i, t} \sim \mathcal{N}(\beta \rmx_{i-1\mod N, t-5}; \sigma^2)$, where $\beta=0.9$ and $\sigma=0.5 ^2$. (b) We name the second dataset "Correlated Sinusoids", inspired by the Discrete Sine Transformation we generate arbitrary signals as the sum of different sinusoids plus gaussian noise. The gaussian noise is independently added to each time series $i$ but the same sinusoid can be shared among different nodes creating strong dependencies. We define different clusters of nodes based on their dependencies, as an example, the first Correlated Sinusoids column in Figure \ref{fig:inference_results} has $N=10$ nodes and two clusters of $5$ nodes each $C=\{5,5\}$, the dataset in the last column has $N=250$ nodes with clusters ranging from size 1 to 22 such that $C=\{1, \dots, 22\}$. Further details and visualizations of these two datasets are provided in Appendix \ref{ap:inferred_graph_datasets}. Both BP-GNN and FC-GNN consist of a single graph convolution from which adjacencies are obtained. We forecast the next time step into the future and optimize the MAE during training. Since our graph inference mechanism is dynamic we average them over 10 timesteps $t$. Further implementation details are described in Appendix \ref{ap:inference_implementation_details}. 


%For BP-GNN we construct the adjacencies as the first N rows and columns of $\tilde{A}=A_2 A_1$ (Eq. \ref{eq:bp_adjacencies}, Sec. \ref{sec:method}). Notice that small K values in BP-GNN may enforce sharing auxiliary nodes and in consequence a more dense adjacency $\tilde{A}$. Further implementation details are described in Appendix \ref{ap:inference_implementation_details}.



\textbf{Results} are reported in Figure \ref{fig:inference_results} for different synthetic datasets which nodes range from $N=10$ to $N=250$. FC-GNN perfectly infers the ground truth adjacencies in all reported datasets and it also achieves the lowest MAE test loss. For the inferred adjacency matrices in BP-GNN, it is harder to develop a visual intuition given the auxiliary nodes, so we omit them from our exposition. However, note that overall accuracy is on par with FC-GNN (specially for datasets with a dense adjacency) and much improved when compared to NE-GNN. So, BP-GNN allows to leverage cross-time series information effectively. Additionally, we also provide visualizations of the inferred graphs in METR-LA in Appendix \ref{ap:inferred_metrla} where we demonstrate the dynamic inference behavior of the graph by plotting the inferred adjacency at different time steps $t$.


\subsection{Choosing the number of auxiliary nodes K} \label{sec:scalability}
In all previous sections we set a relatively small number of auxiliary nodes ($K=4$) for BP-GNN. In this section we analyze the BP-GNN performance as we sweep over different $K$ values  (Figure \ref{fig:sweep_k}). We noticed that for sparser graph datasets as "Cycle Graph", increasing $K$ benefits more than in less sparse graph datasets. In practice, in previous experiments, we chose $K$ to be relatively small since in real world datasets as METR-LA, small $K$ values already provide competitive accuracy with a good trade-off in complexity.

\vspace{-5pt}
\begin{figure}[h!]
\center
\includegraphics[width=0.95\linewidth]{figures/sweep_k.png}
\vspace{-5pt}
\caption{Left: MAE in METR-LA when sweeping $K$ from 0 to 32 auxiliary nodes (10 runs average). Right: MAE in Cycle Graph N=10, when sweeping $K$ from 1 to 10 (4 runs average).}
\label{fig:sweep_k}
\vspace{-3pt}
\end{figure}


\subsection{Complexity analysis}

In Figure \ref{fig:complexity} we provide a visual comparison of the scalability of FC-GNN and BP-GNN (K=4). The right plot shows the vast difference in the number of edges between both methods as we increase the number of nodes. The left plot shows how this translates to the forward time in seconds in the experiments from Section \ref{sec:single_step}.
\vspace{-10pt}
\begin{figure}[h!]
\center
\includegraphics[width=0.95\linewidth]{figures/complexity_analysis.png}
\vspace{-5pt}
\caption{Left: Forward time in seconds for FC-GNN and BP-GNN on different datasets. Right: Scalability of the number of edges w.r.t. the number of nodes $N$.}
\label{fig:complexity}
\vspace{-10pt}
\end{figure}





==> ICML - Time Series Forecasting (6)/sections/introduction.tex <==
%%!TEX root = ../example_paper.tex

\section{Introduction}
Time Series Forecasting (TSF) has been widely studied due to its practical significance in a variety of applications such as climate modelling \citep{mudelsee2019trend}, supply chain management in retail \citep{larson2001designing,bose2017probabilistic}, market analysis in finance \citep{andersen2005volatility}, traffic control \citep{li2017diffusion} and medicine \citep{kaushik2020ai} among others. %\citet{petropoulos2020forecastinglong} provide a non-systematic overview of further applications. 
In TSF, given a sequence of data points indexed over time, we aim to estimate its future values based on previously observed data. Data is often multivariate, meaning that multiple variables vary over time, each variable may not only depend on its own historical values, but also on other variables' past. Efficiently modelling the dependencies among these variables is still an open problem. \vspace{10pt}

Multivariate Time Series (MTS) methods aim to leverage dependencies between variables in order to improve the forecasting accuracy. 
%Some classical MTS forecasting algorithms such as Vector Autoregression (VAR) \citep{lutkepohl2005new} or Gaussian Processes \citep{roberts2013gaussian} only consider linear dependencies among variables. 
A natural way to model non-linear dependencies in deep learning is via Graph Neural Networks (GNNs) \citep{bruna2013spectral, defferrard2016convolutional, kipf2016semi}. In fact, GNNs have been successfully applied to MTS forecasting \citep{li2017diffusion, yu2017spatio, chen2020multi}, leveraging the relations among different series. But these methods require a pre-defined adjacency matrix which may only be available in some specific datasets, for example, traffic datasets, where it can be constructed from the spatial structure of a city. More recently, a family of methods that do not require a pre-defined adjacency matrix have been proposed \citep{wu2019graph, franceschi2019learning, wu2020connecting, shang2021discrete}. In this case, a latent graph representation is inferred while forecasting, allowing to operate on a larger variety of datasets. Our work belongs to this category. 

However, inferring all pairwise relations may come at a higher computational cost, as the number of relations scales quadratically $O(N^2) $ w.r.t. the number of nodes/time series. This limits the scalability to large datasets. Additionally, the above mentioned latent graph inference methods perform message passing updates at every time step iteration which is also expensive. 

To overcome these limitations, we propose a new latent graph inference algorithm for MTS forecasting that is more efficient than previous algorithms while achieving better or competitive performance. We cast the latent graph inference as a modular and easy-to-implement extension to current univariate models. The graph is dynamically inferred for each time series input allowing a more flexible representation than a static graph for the whole dataset. Additionally, we can reduce the complexity from $O(N^2)$ (Fully Connected Assumption) to $O(NK)$ (Bipartite Assumption) where $K \ll N$ for a small trade off in performance.





==> ICML - Time Series Forecasting (6)/sections/method.tex <==
%%!TEX root = ../example_paper.tex

\section{Method} \label{sec:method}

\begin{figure*}[t]
\center
\includegraphics[width=0.9\linewidth]{figures/bipartite_graph_model.jpg}
\caption{Illustration of the presented method under fully connected and bipartite graph assumptions.}
\label{fig:main_model}
\end{figure*}

%\textbf{Model overview}

In Section \ref{sec:background_tsf} we discussed two families of forecasting methods: Global Univariate Models and Multivariate Models. We cast our multivariate algorithm as a modular extension of the univariate case from ~\shorteqref{eq:univariate}. We can break down the Univariate Model in two main steps $f_u = f_{enc} \circ f_{dec}$ such that $\rmx_{i,t_0:t} \stackrel{f_\text{enc }}{\longrightarrow} \rmz_i \stackrel{f_\text{dec }}{\longrightarrow} \hat{\rmx}_{i,t+1:T}$, where $f_{\text{enc}}$ encodes the input signal $\rmx_{i, t_0, t}$ (and optionally some context information $\rmc_i$) into an embedding $\rmz_i$, and $f_\text{dec }$ estimates the future signal from this embedding. In our method, we include a multivariate aggregation module $\mathrm{AGG}$ in between $f_{enc}$ and $f_{dec}$ that propagates information among nodes in the latent space $\rmz = \{\rmz_1, \dots, \rmz_N \}$. This aggregation module takes as input the embedding $\rmz_{i}=f_{enc}( \rmx_{i,t_0:t}, \rmc_i)$, and outputs a modified embedding $\hat{\rmz} = \mathrm{AGG}(\rmz)$ where information has been propagated among nodes. These new embeddings are then passed as input to the decoder $f_{dec}$. The resulting algorithm is:
\begin{align}
    \text{Univariate Encoder}\quad & \rmz_{i}=f_{enc}( \rmx_{i,t_0:t}, \rmc_i) \label{eq:model_encoder}\\
   \text{Multivariate extension}\quad & \hat{\rmz} = \mathrm{AGG}(\rmz) \label{eq:model_aggr} \\
   \text{Univariate Decoder}\quad & \hat{\rmx}_{i, t+1:T} = f_{dec}(\hat{\rmz}_i) \label{eq:model_dec}
\end{align}
Notice the overall model is multivariate but $f_{enc}$ and $f_{dec}$ remain univariate, allowing a modular extension from current univariate methods to multivariate. Additionally, in contrast to the most recent methods \citep{wu2020connecting, shang2021discrete}, our model does not propagate information among nodes at every time step $[t_0,\dots, t]$ but only in the $\mathrm{AGG}$ module. This makes the algorithm cheaper since the message propagation step is usually an expensive operation. Additionally, we experimented including a unique identifier of the time series in the encoded signal $\rmz_i$ as context information $\rmc_i = \text{id}$, which resulted in a significant improvement in accuracy as we will show in the experiments section. In the following subsections we propose two different GNN configurations for the $\mathrm{AGG}$ module depending on the assumed structure of the inferred graph. One is a potentially fully connected graph and the other is a bipartite graph that communicates the N time series through a small set of $K$ auxiliary nodes that we introduce, each has its benefits and weaknesses regarding performance and scalability.  An illustration of the whole algorithm is presented in Figure \ref{fig:main_model}.

\textbf{Fully connected graph assumption | FC-GNN}

From the two configurations, this is the most straightforward to implement given a standard GNN. It results in good performance, but its complexity scales $O(N^2)$ with respect to the number of nodes $N$. Despite this, it still resulted in faster computation times than previous $O(N^2)$ methods.
We can start by defining a fully connected graph $\mathcal{G} = \{\mathcal{V}, \mathcal{E}\}$ where all nodes exchange messages among each other such that $e_{ij}=1$ for all $e_{ij} \in \mathcal{E}$. Each time series embedding $\rmz_i$ obtained from the Univariate Encoder~\shorteqref{eq:model_encoder} is associated with a node of the graph $v_i \in \mathcal{V}$. Then, we can directly use the GNN defined in Section~\shorteqref{sec:background_gnns} as the aggregation module $\mathrm{AGG}$ where each embedding $\rmz_i$ is provided as the input $\rmh_i^0$ to to the GNN~\shorteqref{eq:gnn}, after the GNN runs for $L$ layers, the output node embedding $\rmh^L_i$ is provided as the input $\hat{\rmz}_i$ to the Univariate Decoder~\shorteqref{eq:model_dec}. Moreover, despite the fully connected assumption, the GNN infers attention weights $\alpha_{ij} \in (0, 1)$ \shorteqref{eq:gnn} for each edge and input sample that "gate" the exchanged messages $\rmm_i = \sum_{i \neq j}\alpha_{ij}\rmm_{ij}$. This can be interpreted as dynamically inferring the graph. The reason is that in GNNs we can write the message aggregation as $\rmm_i = \sum_{j \in \mathcal{N}(i)} \rmm_{ij}=\sum_{j  \neq j} e_{ij}\rmm_{ij}$ where $e_{ij}$ is 1 if the edge exists or 0 otherwise. We can see that the following expressions $\sum_{i \neq j}e_{ij}\rmm_{ij} \approx  \sum_{i \neq j}\alpha_{ij}\rmm_{ij}$ becomes equivalent when the soft estimation $\alpha_{ij}=\phi_\alpha(\rmm_{ij})$ approximates/infers the underlying graph $e_{ij}$ structure from the data. In the experiments section, we name this model a Fully Connected Graph Neural Network (FC-GNN). %In summary, the aggregation module $\mathrm{AGG}$ under this FC-GNN assumption, is able to model non-linear relations among time series by exchanging pairwise messages $\rmm_{ij}$~\shorteqref{eq:gnn} among them and inferring the "edges" $\alpha_{ij}$.


\textbf{Bipartite graph assumption | BP-GNN}

In the previous section we presented a GNN method that exchanges information among time series under a fully connected graph assumption which computationally scales $O(N^2)$. In this section we introduce a bipartite graph assumption (BP-GNN) which reduces the complexity to $O(N K)$, $K$ being a parameter of choice $K \ll N$. To accomplish this, we define a bipartite graph $\mathcal{G} = (\mathcal{Y}, \mathcal{U}, \mathcal{E})$, where $\mathcal{Y}$ is a set of $N$ nodes corresponding to the $N$ time series and $\mathcal{U}$ is a set of $K$ auxiliary nodes. Nodes $\mathcal{Y}$ have associated the time series embeddings $\rmz = \{\rmz_1, \dots \rmz_N\}$ and auxiliary nodes $\mathcal{U}$ have associated the embeddings $\rmu = \{\rmu_1, \dots \rmu_K\}$ which are free learnable parameters initialized as gaussian. Edges $\mathcal{E}$ interconnect all nodes between the two subsets $\{\mathcal{Y}$, $\mathcal{U}\}$, but there are no connections among nodes within the same subset. This results in $2NK$ edges.


The message passing scheme works in the following way. We input into the GNN the union of the two node subsets $\mathcal{V} = \mathcal{Y} \cup \mathcal{U}$. Specifically, the input embedding $\rmh^0$ defined in Equation \ref{eq:gnn} is the concatenation of the  time series embeddings $\rmz$ with the auxiliary node embeddings $\rmu$ (i.e. $\rmh^0 = \rmz || \rmu$). Then, messages follow an asynchronous schedule, first information is propagated from the times series nodes to the auxiliary nodes $\mathcal{Y} \xrightarrow{} \mathcal{U}$, next the other way around $\mathcal{U} \xrightarrow{} \mathcal{Y}$.


\begin{table}[h] \small
\setlength{\tabcolsep}{3pt}
\begin{center} 
\begin{tabular}{c|c}
\toprule
Step 1 & Step 2\\
$\mathcal{Y} \rightarrow \mathcal{U}$ & $\mathcal{U} \rightarrow \mathcal{Y}$ \\
\midrule 
$i \in \mathcal{U} \quad , \quad j \in \mathcal{Y}$ & $i \in \mathcal{Y} \quad , \quad j \in \mathcal{U}$\\
\midrule
\begin{math}
\begin{aligned}
\rmm_{ij} &= \phi_{e_1}(\rmh_i^l, \rmh_j^l, a_{ij}) \\
    \rmm_i &= {\textstyle \sum_{j \in \mathcal{Y}} \phi_{\alpha_1}(\rmm_{i j})\rmm_{i j}} \\
    \rmh_i^{l+1} &= \phi_{h_1}(\rmh_i^l, \rmm_i) \\
\end{aligned}
\end{math}
 &
 \begin{math}
\begin{aligned}
\rmm_{ij} &= \phi_{e_2}(\rmh_i^l, \rmh_j^l, a_{ij}) \\
    \rmm_i &= {\textstyle \sum_{j \in \mathcal{U}}} \phi_{\alpha_2}(\rmm_{i j})\rmm_{i j} \\
    \rmh_i^{l+1} &= \phi_{h_2}(\rmh_i^l, \rmm_i) \\
\end{aligned}
\end{math}\\
\bottomrule
\end{tabular}
\caption{BP-GNN formulation.}
\label{tab:eq_bp} 
\end{center}
\vspace{-12pt}
\end{table}


We have conceptually defined the Bipartite Graph Neural Network. In Table \ref{tab:eq_bp} we introduce the equations that formally define it as an extension of the standard GNN Equation
\ref{eq:gnn}. Notice that it can be simply formulated as a two steps process where the indexes $i,j$ belong to each one of the subsets $\mathcal{U}$ or $\mathcal{Y}$ depending on the direction of the messages ($\mathcal{Y} \rightarrow \mathcal{U}$ or $\mathcal{U} \rightarrow \mathcal{Y}$). Additionally, we used different learnable parameters between Step 1 and Step 2 in the modules $\phi_e$, $\phi_{\alpha}$ and $\phi_h$ since it resulted in better performance than sharing parameters. Following, we define the adjacency matrices corresponding to the two message passing steps (assuming all inference parameters $\alpha_{ij} = 1$):

\begin{equation}
\small
  A_1 =  \begin{vmatrix} 
    0_{N \times N} & 0_{N \times K}   \\
   1_{K \times N} & 0_{K \times K} \\
   \end{vmatrix} 
,\quad
  A_2 =  \begin{vmatrix} 
  0_{N \times N} & 1_{N \times K}   \\
   0_{K \times N} & 0_{K \times K} \\
   \end{vmatrix}
       \label{eq:bp_adjacencies}
\end{equation}



$A_1$ refers to $\mathcal{Y} \xrightarrow{} \mathcal{U}$ and $A_2$ refers to $\mathcal{U} \xrightarrow{} \mathcal{Y}$. The product of these two matrices $\tilde{A} = A_2A_1$ (Appendix \ref{eq:bp_adjacencies}) defines the sum of all paths that communicate the time series nodes $\mathcal{Y}$ among each other through the auxiliary nodes $\mathcal{U}$. Notice that for $K>0$ all nodes $\mathcal{Y}$ can potentially communicate among them being more efficient than FC-GNN as long as $0  \leq K < N/2$.








%\textbf{Scaling the GNN to larger graphs | Bipartite graph}

%The presented model that infers the edges scales computationally $O(N^2)$ with respect to the number of nodes. In the end the final goal of that module is to exchange information among nodes but they do not need to be all connected with each other. We can actually define a set of $K$ latent nodes $\rmb = {\rmb_1, \dots, \rmb_K}$ that together with $\rmh$ define a bipartite graph of $N \cdot K$ nodes. But since it is a bipartite graph there are only existing edges between the two subsets $\rmh$ and $\bvec$ but not between elements of the same subset. The computation complexity is then reduced to $O(N\cdot K)$.



%More formally, the new graph nodes would be defined as $\hat{\mathbf{h}} = \mathbf{h} \mathbin\Vert \mathbf{b}$ where $\hat{\mathbf{h}}$ has $N + K$ nodes. The adjacency matrix will then be limited to connections between the nodes $\rmh$ and $\rmb$:


%\begin{equation}
%  A =  \begin{vmatrix} 
%   0_{N \times N} & 1_{N \times K}   \\
%   (1_{K \times N})^T & 0_{K \times K} \\
%   \end{vmatrix} 
%\end{equation}

%Notice that by just jumping two steps away we get again a fully connected graph, but since we are factorizing it in two different time steps the coplexity is reduced from $O(N^2)$ to $O(2  N  K)$, where $K$ can be any arbitrary value although it can depend on $N$ for a certain approximation error. 

%\begin{equation}
%  A_{fc}=A \cdot A =  \begin{vmatrix} 
%   K_{N\times N} & 0   \\
%   0 & N_{K\times K}\\
%   \end{vmatrix} 
%\end{equation}


%\textbf{Scaling the GNN to larger graphs | Bipartite asynchronous graph}

%We perform two different message passing updates from the time series nodes to the latent nodes and vice-versa.





%\begin{equation}
%  A_a =  \begin{vmatrix} 
%   0_{N \times N} & 1_{N \times K}   \\
%   0_{K \times N} & 0_{K \times K} \\
%   \end{vmatrix} 
%\end{equation}

%\begin{equation}
%  A_b =  \begin{vmatrix} 
%   0_{N \times N} & 0_{N \times K}   \\
%   1_{K \times N} & 0_{K \times K} \\
%   \end{vmatrix} 
%\end{equation}

%After these two message passing updates each time series receives information from all other time series but the number of edges is $2 NK$ instead of $NN$


%\begin{equation}
%  A = A_aA_b =  \begin{vmatrix} 
%   K_{N \times N} & 0_{N \times K}   \\
%   0_{K \times N} & 0_{K \times K} \\
%   \end{vmatrix} 
%\end{equation}

% We can choose $K$


%\textbf{Scaling the GNN to larger graphs | Sparsity}

%Another alternative way to scale the graph to larger graphs would be removing edge connections at random from the fully connected graph that scaled $O(N^2)$. We call it \textit{SparseGNN}.



%{\color{red} This method performs well, but sparsity is introduced at random. It would be interesting to learn the sparsity from the dataset and then fine-tune it with attention}


\textbf{Architecture details}

Recall that our method is composed of three main modules, the encoder $f_{enc}$, the decoder $f_{dec}$ and the aggregation module $\mathrm{AGG}$. We choose to use relatively simple networks as encoder and decoder. The decoder $f_{dec}$ is defined as a Multi Layer Perceptron (MLP) with a single hidden layer and a residual connection in all experiments. The encoder $f_{enc}$ is also defined as an MLP for METR-LA, PEMS-BAY and our synthetic datasets and as a Convolutional Neural Network (CNN) for the other datasets since these require a larger encoding length and the translation equivariance of CNNs showed to be more beneficial. The encoder $f_{enc}$, first encodes the input signal $\rmx_{i, t_0:t}$ to an embedding vector by using the mentioned MLP or CNN, and then concatenates a unique identifier ($\rmc_i = \text{id}$) to the obtained embedding vector resulting in $\rmz_i$. $\rmc_i$ could (optionally) include additional context information if it was provided in the dataset. The combination of these simple networks with our proposed aggregation module $\mathrm{AGG}$ fully defines our model. 

The aggregation module $\mathrm{AGG}$ was defined under two different assumptions, the Fully Connected Graph assumption (FC-GNN) and the Bipartite Graph assumption (BG-GNN). In both cases the GNN is fully parametrized by the networks 
$\phi_e$, $\phi_h$ and $\phi_\alpha$. $\phi_e$ consists of a two layers MLP, $\phi_h$ is a one layer MLP with a skip connection from he input to the output and $\phi_\alpha$ is just a linear layer followed by a Sigmoid activation function.
 All architecture choices are explained in more detail in Appendix~\ref{ap:architecture_choices}. 
We optimized the Mean Absolute Error as the loss $\mathcal{L}=l(\hat{\rmx}_{ t+1:T}, \rmx_{t+1:T})$ for training.

%\textbf{From graph to hierarchies}

%In this section we show the relations of the graph structured representations with hierarchical representations. We show that hierarchical representations are a particular solution of the bipartite graph representation.

==> ICML - Time Series Forecasting (6)/sections/related_work.tex <==
%%!TEX root = ../example_paper.tex

\section{Related Work}
Time series forecasting has been extensively studied in the past due to its practical significance with a number of recent overview articles available~\citep{petropoulos2020forecasting,overview20,Lim_2021}. Traditionally, most classical methods are univariate in nature (see e.g.,~\cite{hyndman2017forecasting} for an overview). While some of these have multi-variate extensions (e.g., ARMA and VARMA models), they are limited by the amount of related time series information they can incorporate. Dynamic factor models \citep{geweke1977dynamic, wang2019deepfactors} are fore-runners of a family of models that has recently received more attention, the so-called global models \citep{januschowski19,montero2020principles}, see Section~\ref{sec:background_tsf}. These global models estimate their parameters over an entire panel of time series, %so thereby taking advantage of cross time series learning, 
but still produce a univariate forecast. Many such global models have been proposed building on neural network architectures like RNNs~\citep{salinas2020deepar,Liberty2020,kasun19}, CNNs~\citep{wen2017multi,chen2019probabilistic}, Transformers~\citep{li2019neurips,lim2021temporal,eisenach2020mqtransformer} and also combining classical probabilistic models with deep learning \citep{rangapuram2018deep,kurle2020deep,de2020normalizing}.  However, unlike our method, these global models do not explicitly model the relationship between the time series in the panel.

Most recently, global multi-variate forecasting models have received attention, in particular models that attempt to capture the relationship of the time series via a multi-variate likelihood \citep{rasul2020multi,rasul2021autoregressive,de2020normalizing,multivariate19}. A complementary approach consists of capturing the multi-variate nature of many modern forecasting problems primarily by using a multi-variate time series as input. For this, a natural way to model and exploit the relationship between time series is via GNNs~\citep{bruna2013spectral, defferrard2016convolutional, kipf2016semi}. Even in those scenarios where the adjacency of the graph is explicitly provided, attention or a latent graph can be inferred from the node embeddings such that GNNs can still leverage the structure of the data. Some examples of latent graph inference or attention are \citep{wang2019dynamic} in point clouds, \citep{franceschi2019learning} in semi-supervised graph classification,  \citep{ying2018hierarchical} in hierarchical graph representation learning, \citep{kipf2018neural} in modelling dynamical systems, \citep{kazi2020differentiable} in zero-shot learning and 3D point cloud segmentation, \citep{garcia2017few, kossen2021self} in image classification, \citep{cranmer2020discovering} in inferring symbolic representations and \citep{fuchs2020se, satorras2021n} in molecular property prediction.

In MTS forecasting, \citet{lai2018modeling,shih2019temporal} provide some of the first deep learning approaches designed to leverage pair-wise dependencies among time series. More recent methods~\citep{li2017diffusion,yu2017spatio,seo2018structured,zhao2019t} are built in the intersection of GNNs and time series forecasting but they require a pre-defined adjacency matrix. Lately, new methods that infer a latent graph from the node embeddings have been introduced in MTS forecasting \citep{wu2020connecting, shang2021discrete, cao2021spectral}, and in MTS anomaly detection \citep{zhang2020correlation, deng2021graph}. These methods can be applied to any dataset even when there is not an explicitly defined adjacency matrix. The main limitation is the computational cost, which occurs in the edge inference and scales quadratically $O(N^2)$  w.r.t the number of nodes/time series $N$ or $O(N^3)$ in \citep{wu2020connecting, cao2021spectral}. 


Our approach is related to \citep{wu2020connecting, shang2021discrete}, but in contrast (i) our latent graph is dynamically inferred for each input instead of static for the whole dataset; (ii) it only requires the message exchange at time step $t$ which renders the graph operation cheaper and modular; and (iii) it optionally reduces the number of edges from $O(N^2)$ to $O(NK)$ when using a bipartite assumption ($K \ll N$).

\paragraph{Linear vs Non-linear message passing} 
A shared potential limitation among the mentioned methods that use GNNs for MTS Forecasting \citep{yu2017spatio, li2017diffusion, seo2018structured, zhao2019t, wu2019graph, wu2020connecting, shang2021discrete, cao2021spectral} is the use of a linear function in the edge operation \citep{defferrard2016convolutional, kipf2016semi}. In contrast, we allow for non-linearities in our model.  Table~\ref{tab:gnns_comparison} provides an overview comparing these two alternatives by writing the linear graph convolutional layer in the same format as the non-linear one \citep{gilmer2017neural} from Section \ref{sec:background_gnns}. Where $\theta_e,\theta_h \in \mathbb{R}^{\text{nf} \times \text{nf}}$ are learnable parameters.

\vspace{-4pt}
\begin{table}[h!]
\footnotesize
%\setlength{\tabcolsep}{2pt}
\begin{center} 
\begin{tabular}{ c  c c } 
\toprule
  & Non-linear & Linear\\
  \midrule
  Edge & $\rmm_{ij} = \phi_e(\rmh_i^l, \rmh_j^l)$ & $\rmm_{ij} = \mathbf{\theta}_e^\intercal \rmh_j $ \\
  \midrule
Aggr &  \multicolumn{2}{c }{$\rmm_i = \sum_{j \in \mathcal{N}(i)} \rmm_{i j}$} \\

  \midrule
    % \midrule
  Node & $\rmh_i^{l+1} = \phi_h(\rmh_i^l, \rmm_i) $ & $\rmh_i^{l+1}  =  \sigma(\rmm_i + \theta_h^\intercal\rmh_h^l) $  \\

    \bottomrule
\end{tabular}
\vspace{-3pt}
\caption{Non-linear vs Linear Graph Conv. Layer comparison.}
\label{tab:gnns_comparison} 
\end{center}
\vspace{-14pt}
\end{table}

The linear graph convolutional layer is commonly written in matrix form as we show in Appendix~\ref{ap:linear_graph}. Note that while the non-linear alternative approximates the edge operation with an MLP $\phi_e$, in the linear case the message operation among two nodes ($i,j$) only depends on node $\rmh_j$ and it is agnostic to the identity of the receiver node $i$. This can be problematic when inferring relations among two nodes since the message operation only depends on one of them. Therefore, when no adjacency matrix is provided, an attention mechanism that depends on both $i,j$ can address some of these limitations $\rmm_{ij}= \alpha(i,j) \theta_e^\intercal \mathbf{h}_j$. However, note that in the non-linear case, $\phi_e$ is a universal approximator that can be interpreted as a generalization of the linear case with attention ${\phi}_e(\rmh_i, \rmh_j) = \alpha(i,j) \theta_e^\intercal \mathbf{h}_j$. In practice, even if the non-linear case can more flexibly model $\rmm_{ij}$, it has been shown in previous literature that attention or edge inference \citep{vaswani2017attention, satorras2021n} can be a strong inductive bias which in our case is able to infer the graph structure as we will show in the experiments section.


%(GTS and MTGNN) These two models learn an adjacency matrix which scales computationally $O(N^2)$. Our method performs competitively or better while it scales $O(NK)$. Where $K$ can be fixed or may depend on $N$ for a certain approximation error. In our experiments we analyze the bahavior for different $K$ values and we pick $K=\sqrt{N}$ for most experiments since it didn't produce a decrease in performance.
